Low-Autocorrelation Binary Sequences: On Improved Merit Factors and Runtime Predictions to Achieve Them

The search for binary sequences with a high figure of merit, known as the low autocorrelation binary sequence ($labs$}) problem, represents a formidable computational challenge. To mitigate the computational constraints of the problem, we consider solvers that accept odd values of sequence length $L$ and return solutions for skew-symmetric binary sequences only -- with the consequence that not all best solutions under this constraint will be optimal for each $L$. In order to improve both, the search for best merit factor $and$ the asymptotic runtime performance, we instrumented three stochastic solvers, the first two are state-of-the-art solvers that rely on variants of memetic and tabu search ($lssMAts$ and $lssRRts$), the third solver ($lssOrel$) organizes the search as a sequence of independent contiguous self-avoiding walk segments. By adapting a rigorous statistical methodology to performance testing of all three combinatorial solvers, experiments show that the solver with the best asymptotic average-case performance, $lssOrel\_8 = 0.000032*1.1504^L$, has the best chance of finding solutions that improve, as $L$ increases, figures of merit reported to date. The same methodology can be applied to engineering new $labs$ solvers that may return merit factors even closer to the conjectured asymptotic value of 12.3248.

==> Figures/fg_known_merit_factors_from_literature.tex <==
\begin{figure*}
\centering 
\subfloat[]{
\begin{minipage}{0.99\textwidth}
\renewcommand{\arraystretch}{0.9}
\centering
\begin{footnotesize}
\begin{tabular}{c|c c c c c c c c c | r r r }
	{\bf L} & \cite{Lib-OPUS-labs-1985-Phillips-Beenker} & \cite{Lib-OPUS-labs-1990-IEEE_TIT-Golay-skewsym} & 
	\cite{Lib-OPUS-labs-1993-Diploma-Reinholz-genetic-alg} & \cite{Lib-OPUS-labs-2007-Prestwich-local-search} & \cite{Lib-OPUS-labs-1998-IEEE_EC-Militzer} &
	\cite{Lib-OPUS2-labs-2014-homepage-Knauer} & \cite{Lib-OPUS-labs-2008-LMSLNS-Borwein}& \cite{Lib-OPUS-labs-2009-ASC-Gallardo-memetic} & 
	{\bf \lssOrelE} & $\lceil 100*{\cal H}_{obs} \rceil$ & $m_{L}$ & $\Delta (E)$\\
	\hline \\[-1.8ex]
	107 & 6.53 & {\bf 8.46} & {\bf 8.46} & 8.36 & {\bf 8.46} & {\bf 8.4557} & - & {\bf 8.4557} & {\bf 8.4557} & 100 & 1 & 0 \\
	109 & 6.15 & {\bf 8.97} & {\bf 8.97} & {\bf 8.97} & {\bf 8.97} & {\bf 8.9736} & - & {\bf 8.9736} & {\bf 8.9736} & 100 & 1 & 0 \\
	111 & 6.02 & {\bf 8.97} & {\bf 8.97} & {\bf 8.97} & {\bf 8.97} & {\bf 8.9672} & - & {\bf 8.9672} & {\bf 8.9672} & 100 & 1 &  0\\
	113 & 6.33 & {\bf 8.49} & {\bf 8.49} & {\bf 8.49} & {\bf 8.49} & {\bf 8.4900} & - & {\bf 8.4900} & {\bf 8.4900} & 100 & 2 & 0\\
	115 & 6.40 & {\bf 8.88} & 8.60 & {\bf 8.88} & {\bf 8.88} & {\bf 8.8758} & - &  {\bf 8.8758} & {\bf 8.8758} & 100 & 1 & 0\\
	117 & 6.42 & {\bf 8.71} & 8.12 & {\bf 8.71} & {\bf 8.71} & {\bf 8.7080} & - & {\bf 8.7080} & {\bf 8.7080} & 100 & 1 & 0\\
	119 & 6.01 & - & 7.67 & {\bf 8.48} & 8.02 & {\bf 8.4796} & - & {\bf 8.4796} & {\bf 8.4796} & 100 & 1 & 0\\
	121 & 6.61 & - & {\bf 8.67} & - & {\bf 8.67} & {\bf 8.6736} & - &  {\bf 8.6736} & {\bf 8.6736} & 100 & 1 & 0\\
	141 & 6.01 & - & 7.45 & - & {\bf 8.83} & {\bf 8.8282} & - & {\bf 8.8282} & {\bf 8.8282} & 100 & 2 & 0\\
	149 & - & - & - & - & - & {\bf 9.1137} &  {\bf 9.1137} & - & {\bf 9.1137} & 95 & 1 & 0\\
	157 & - & - & - & - & - & {\bf 9.0223} &  {\bf 9.0223} & - & {\bf 9.0223} & 98 & 1 & 0\\
	161 & 6.02 & - & 6.89 & - & 8.39 & 8.5266 & - & {\bf 8.5718} & {\bf 8.5718} & 76 & 2 & 0\\
	165 & - & - & - & - & - & {\bf 9.2351} &  {\bf 9.2351} & - & {\bf 9.2351} & 26 & 1 & 0\\
	169 & - & - & - & - & - & {\bf 9.3215} &  {\bf 9.3215} & - & {\bf 9.3215} & 24 & 1 & 0\\
	173 & - & - & - & - & - & 9.3179 &  {\bf 9.3645} & - & {\bf 9.3645} & 28 & 1 & 0\\
	175 & - & - & - & - & - & 8.9078 &  {\bf 9.0768} & - & {\bf 9.0768} & 12 & 1 & 0\\
	177 & - & - & - & - & - & 8.6640 &  {\bf 9.5052} & - & {\bf 9.5052} & 10 & 1 & 0\\
	179 & - & - & - & - & - & 8.4452 &  {\bf 9.0974} & - & {\bf 9.0974} & 6 & 1 & 0\\
	181 & 7.70 & - & 6.77 & - & 7.75 & 8.6304 & - & 7.7194 & {\bf 8.9316} & 6 & 1 & 64 \\
	183 & - & - & - & - & - & 8.3932 &  {\bf 9.0073} & - & {\bf 9.0073} & 5 & 2 & 0 \\
	189 & - & - & - & - & - & {\bf 9.0847} &  {\bf 9.0847} & - & {\bf 9.0847} & 1 & 1 & 0\\
	201 & - & - & 6.29 & - & 7.46 & 8.2116 & - &  7.6633 & {\bf 8.4876} & 1 & 1 & 80\\
	215 & - & - & - & - & - & ~$8.1641^{*}$ & - & - & {\bf 8.5888} & 1 & 1 & 140\\
	221 & - & - & - & - & - & 7.6171 & - & - & {\bf 8.8544} & 1 & 1 & 448\\
	241 & - & - & - & - & - & 7.2747 & - &  - & {\bf 8.0668} & 1 & 1 & 392\\
	249 & - & - & - & - & - & ~$7.2431^{*}$ & - & - & {\bf 8.1323} & 1 & 1 & 468\\
	259 & - & - & - & - & - & ~$7.1287^{*}$ & - & - & {\bf 8.0918} & 1 & 1 & 560\\
	261 & - & - & - & - & - & ~$7.1108^{*}$ & - & - & {\bf 7.8517} & 1 & 1 & 452\\
	271 & - & - & - & - & - & ~$7.0037^{*}$ & - & - & {\bf 7.5386} & 1 & 1 & 372\\
	281 & - & - & - & - & - & 7.0957 & - & - & {\bf 7.5058} & 1 & 1 & 304\\
	283 & - & - & - & - & - & ~$7.0291^{*}$ & - & - & {\bf  7.5088} & 1 & 1 & 364\\
	301 & - & - & - & - & - & - & - & - & {\bf  7.4827} & 1 & 1 & - \\
	303 & - & - & - & - & - & 7.1115 & - & - & {\bf 7.2462} & 1 & 1 & 120 \\
	341 & - & - & - & - & - & - & - & - & {\bf 6.9397} & 1 & 1 & - \\
	381 & - & - & - & - & - & - & - & - & {\bf 7.0893} & 1 & 1 & - \\
	401 & - & - & - & - & - & - & - & - & {\bf 6.7632} & 1 & 1 & -\\
\end{tabular}
\end{footnotesize}
\label{fg_known_merit_factors_from_literature-a}
\end{minipage}
}

\subfloat[]{
\begin{minipage}{0.49\textwidth}
\includegraphics[width=0.99\textwidth]{Figures/fg_histogram_L241-a}
\label{fg_known_merit_factors_from_literature-b}
\end{minipage}
}
\subfloat[]{
\begin{minipage}{0.49\textwidth}
\includegraphics[width=0.99\textwidth]{Figures/fg_histogram_L241-b}
\label{fg_known_merit_factors_from_literature-c}
\end{minipage}
}
\caption{
(a) Comparisons of the best-known merit factors reported in the literature and 
the best-known merit factors obtained by \lssOrelE.
Two views of best merit factors for $L$ = 241 in a special-case experiment with \lssOrelE, 
running on 100 instances for a total of 4 days:
(b) a runtime scatter plot of best merit factors,
(c) a histogram of merit factor frequencies.
}
\label{fg_known_merit_factors_from_literature}
\end{figure*}


==> Figures/fg_model_mean.tex <==
\begin{figure*}[t!]
\vspace*{-6ex}
\centering
\subfloat{
\begin{minipage}{0.49\textwidth}
\includegraphics[width=0.99\textwidth]{Figures/fg_model_mean-a}
\end{minipage}
}
\subfloat{
\begin{minipage}{0.49\textwidth}
\includegraphics[width=0.99\textwidth]{Figures/fg_model_mean-b}
\end{minipage}
}
\vspace*{-4ex}
\subfloat{
\begin{minipage}[]{0.49\textwidth}
\includegraphics[width=0.99\textwidth]{Figures/fg_model_mean-c}
\end{minipage}
}
\subfloat{
\begin{minipage}{0.49\textwidth}
\includegraphics[width=0.99\textwidth]{Figures/fg_model_mean-d}
\end{minipage}
}
\caption{
The asymptotic performance of the solver \lssOrelU. For each value of $L$
and from each of the 
100 randomly assigned initial coordinates, this solver finds one of the four possible
optimal solution by performing a single
contiguous self-avoiding walk. Examples of variable correlations that 
remain consistently highly correlated throughout our experiments include {\em cntProbe} versus {\em runtime} and {\em walkLength} versus {\em cntProbe}.
The values of $L = \{41, 43, 45, 51, 57, 71, 77, 83, 91, 95, 97, 99, 101, 103, 105\}$ represent the subset hardest-to-solve instances
of the \labs\ problem; see Eq.~\ref{eq_L_primary} and Table~\ref{tb_L_asymptotic}.
The asymptotic predictor model in the form of ($a*b^{L}$) interpolates between 14 sample means, 
each based on a sample size of 100.
Since the solver relies on skew-symmetry formulation of the binary sequence, 
{\em cntProbe} has the following relationship with {\em walkLength}: $cntProbe \approx walkLength * \frac{L+1}{2}$.
}
\label{fg_model_mean}
\end{figure*}




==> Tables/tb_BB-vs-others-asymptotes.tex <==
\begin{table}[t!]
\caption{
Observed/projected asymptotic performance of state-of-the- art branch-and-bound \labs\ solver
under skew-symmetry \cite{Lib-OPUS-labs-2013-arxiv-Prestwich-branch-and-bound-odd} versus the observed/projected
runtime of two stochastic solvers under skew-symmetry: \lssOrelE\ and \lssMAts.
}

\label{tb_BB-vs-others-asymptotes}
\centering
\begin{footnotesize}
 \begin{tabular}{@{~}r@{~}|l l | l l}
  \multirow{2}{*}{L} & \multicolumn{2}{c|}{runtime [years]} & \multicolumn{2}{@{~}c@{~}}{100 $\times$ runtime [years]} \\
 & \multicolumn{1}{c}{BB} 
 & \multicolumn{1}{c|}{ratio$^\dagger$} 
 & \multicolumn{1}{c}{\lssOrelE} 
 & \multicolumn{1}{c}{\lssMAts} \\
  \hline
75 & 1.1590e-04~\, & 3.1194e+03 & 3.7154e-06$^*$ & 3.3649e-06$^+$ \\
77 & 2.8983e-04~\, & 5.7999e+03 & 4.9971e-06~\, & 4.7695e-06~\,\\
79 & 5.6726e-04~\, & 8.7172e+03 & 6.5074e-06$^*$ & 6.3574e-06$^+$ \\
81 & 8.9805e-04~\, & 1.0428e+04 & 8.6120e-06$^*$ & 8.7384e-06$^+$ \\
83 & 1.1310e-03~\, & 2.8420e+03 & 3.9795e-05~\, & 8.5217e-06~\,\\
85 & 2.3780e-03~\, & 1.5766e+04 & 1.5083e-05$^*$ & 1.6510e-05$^+$ \\
87 & 4.5392e-03~\, & 2.2739e+04 & 1.9962e-05$^*$ & 2.2693e-05$^+$ \\
89 & 9.0476e-03~\, & 3.4249e+04 & 5.3345e-06 & 1.0364e-05 \\
115 & 1.5758e+01$^*$ & 1.7756e+06 & 8.8751e-04~\, & 1.8324e-03~\,\\
121 & 9.0011e+01$^*$ & 4.2144e+06 & 2.1358e-03~\, & 4.2444e-03~\,\\
127 & 5.1414e+02$^*$ & 1.0145e+07 & 5.0680e-03~\, & 1.0521e-02~\,\\
141 & 2.9986e+04$^*$ & 7.7784e+07 & 3.8551e-02~\,  & 1.2189e-01~\,   \\
151 & 5.4732e+05$^*$ & 3.4972e+08 & 1.5650e-01$^*$ & 5.9805e-01$^+$ \\
161 & 9.9897e+06$^*$ & 1.5723e+09 & 6.3534e-01$^*$ & 2.9342e+00$^+$ \\
181 & 3.3280e+09$^*$ & 3.1783e+10 & 1.0471e+01$^*$ & 7.0634e+01$^+$ \\
201 & 1.1087e+12$^*$ & 6.4245e+11& 1.7257e+02$^*$ & 1.7003e+03$^+$ \\
241 & 1.2304e+17$^*$ & 2.6322e+14 & 4.6744e+04$^*$ & 9.8259e+05$^+$ \\
\hline
\multicolumn{5}{l}{ }  \\[-1.5ex]
\multicolumn{5}{l}{The unmarked values have been observed experimentally, }  \\
\multicolumn{5}{l}{the values marked with $^*$ and $^+$ are based on predictions below: }  \\
\multicolumn{5}{l}{BB = 1.55311e-06*$1.3370^L/(3600*24*366)$ }  \\
\multicolumn{5}{l}{$^\dagger$~ratio~=~runtime(BB)/runtime(\lssOrelE) }  \\
\multicolumn{5}{l}{$^*~\lssOrelE = 100*(0.000032*1.1504^L/(3600*24*366))$} \\
\multicolumn{5}{l}{$^+~\lssMAts~~~~  = 100*(0.000007*1.1724^L/(3600*24*366))$} \\
\end{tabular}
\end{footnotesize}
\end{table}


==> Tables/tb_predictions.tex <==
\OMIT{
#>>>>>>>>>>>>>>>>>>>
# This calculation is relevant when explaining hitO for L <= 141  AND for L > 141 
# (search for hitO below)
# L = c(83,91,95,97,99,101, 103,105, 107, 109, 111, 115, 117, 119, 121, 123, 125, 127)
# meanRuntime = c(12.54981, 7.78170, 30.52900, 28.55490, 14.34310,34.1979, 48.3007, 69.0639, 446.993, 83.2342, 154.217, 279.885, 299.875, 355.601,673.546,2181.08,1427.5,1598.24)
# tObs=as.integer(meanRuntime) ; tObs
#[1]   12    7   30   28   14   34   48   69  446   83  154  279  299  355  673 2181 1427 1598
# tPred=as.integer(0.000032*1.1504^L) ; tPred
#1]    3   11   19   25   33   44   59   78  103  137  181  318  421  557  737  976 1291 1709
# diff = -tPred + tObs ; diff
#1]    9   -4   11    3  -19  -10  -11   -9  343  -54  -27  -39 -122 -202  -64 1205  136 -111
# cbind(L,tPred, tObs, diff)
#        L tPred tObs diff
#[1,]  83     3   12    9
#[2,]  91    11    7   -4
#[3,]  95    19   30   11
#[4,]  97    25   28    3
#[5,]  99    33   14  -19
#[6,] 101    44   34  -10
#[7,] 103    59   48  -11
#[8,] 105    78   69   -9
#[9,] 107   103  446  343
#[10,] 109   137   83  -54
#[11,] 111   181  154  -27
#[12,] 115   318  279  -39
#[13,] 117   421  299 -122
#[14,] 119   557  355 -202
#[15,] 121   737  673  -64
#[16,] 123   976 2181 1205
#[17,] 125  1291 1427  136
#[18,] 127  1709 1598 -111
# 
# 
#>>>>>>>>>>>>>>>>>>>
}

\begin{table}[h!]
  \caption{ 
  Mean value runtime predictions  
  versus the observed runtime means  with the solver \lssOrelE:
  $\overline{m}(L) = 0.000032*1.1504^L$ versus $\overline{m}_{obs}(L)$.
  For values of $L \le 141$,
  none of the $N=100$ runs are censored within 
  the time limit of $t_{lmt} = 4$  days (345600 seconds),
  hence the observed number of hits is {\em hitO = 100}
  and the reported values of observed runtime means  are within the confidence
  interval defined in Eq.~\ref{eq_confidenceInterval}.
  Relative to the predicted value of $\overline{m}(L)$, the
  ratio of $\overline{m}_{obs}(L)/\overline{m}(L) > 1$
  is an indicator of the instance solvability as well as the level of the landscape 
  {frustration}~\cite{Lib-OPUS-labs-2014-NatNano-frustrated-energy-landscape};
  a property characteristic of the 
  the \labs\ problem. All instances with more than a single canonic solution ($C_L > 1$)
  have been excluded from this prediction model.
}
  \label{tb_predictions}
  \centering
  \begin{small}
 \begin{tabular}{c|c c c c c}
 $L$& $\overline{m}(L)$ & $\overline{m}_{obs}(L)$ & $\Delta(\rm{seconds})$ & ratio & $C_{L}$ \\
 \hline
 83 &   3  &   12 &     9 &  4.00 & 1\\
 91 &   11 &   7  &    -4 & -0.63 & 1\\
 95 &   19 &   30 &    11 &  1.58 & 1\\
 97 &   25 &   28 &     3 &  1.12 & 1\\
 99 &   33 &   14 &   -19 & -0.42 & 1\\
101 &   44 &   34 &   -10 & -0.77 & 1\\
103 &   59 &   48 &   -11 & -0.81 & 1\\
105 &   78 &   69 &    -9 & -0.88 & 1\\
107 &  103 &  446 &   343 &  4.33 & 1\\
109 &  137 &   83 &   -54 & -0.61 & 1\\
111 &  181 &  154 &   -27 & -0.85 & 1\\
115 &  318 &  279 &   -39 & -0.87 & 1\\
117 &  421 &  299 &  -122 & -0.71 & 1\\
119 &  557 &  355 &  -202 & -0.63 & 1\\
121 &  737 &  673 &   -64 & -0.91 & 1\\
123 &  976 & 2181 &  1205 &  2.23 & 1\\
125 & 1291 & 1427 &   136 &  1.11 & 1\\
127 & 1709 & 1598 &  -111 & -0.94 & 1
 \end{tabular}
 \end{small}
\end{table}


==> Tables/tb_runtime_6_34.tex <==
   \begin{table}
    \centering
    \label{runtimes}
    \caption{Runrimes for \lssOrelE\ to obtain merir factor of 6.34 for L bilonging to primer numbers.}
    \begin{tabular}{c | c c c c c c}
     \multirow{2}{*}{L} & \multicolumn{2}{c}{runtime} & \multirow{2}{*}{runs} & \multirow{2}{*}{hits} & \multirow{2}{*}{$m_L$}\\
       & mean & std & \\
     \hline
     151 & 0.998 & 0.878 & 100 & 100 & 100\\
     157 & 1.677 & 1.561 & 100 & 100 & 100\\
     163 & 2.190 & 2.017 & 100 & 100 & 100\\
     167 & 2.738 & 3.183 & 100 & 100 & 100\\
     173 & 3.806 & 3.669 & 100 & 100 & 100\\
     179 & 6.025 & 6.085 & 100 & 100 & 100\\
     181 & 5.318 & 5.644 & 100 & 100 & 100\\
     191 & 10.518 & 8.7613 & 100 & 100 & 100\\
     193 & 12.725 & 10.751 & 100 & 100 & 100\\
     197 & 11.658 & 10.359 & 100 & 100 & 100\\
     199 & 13.113 & 14.898 & 100 & 100 & 100\\
     211 & 24.447 & 27.494 & 100 & 100 & 100\\
     223 & 50.892 & 52.068 & 100 & 100 & 100\\
     227 & 59.673 & 66.783 & 100 & 100 & 100\\
     229 & 62.072 & 51.977 & 100 & 100 & 100\\
     233 & 76.144 & 82.144 & 100 & 100 & 100\\
     239 & 109.536 & 107.367 & 100 & 100 & 100\\
     {\bf 241} & {\bf 102.736} & {\bf 110.403} & {\bf 100} & {\bf 100} & {\bf 100}\\
     {\bf 241} & {\bf 1141.86} & {\bf 1146.81} & {\bf 73} & {\bf 73} & {\bf 73} & {\bf \lssMAts} \\  
     251 & 143.042 & 128.677 & 100 & 100 & 100\\
     257 & 248.972 & 273.954 & 100 & 100 & 100\\
     263 & 267.007 & 259.58 & 100 & 100 & 100\\
     269 & 381.678 & 387.835 & 100 & 100 & 100\\
     271 & 405.055 & 395.192 & 100 & 100 & 100\\
     277 & 570.184 & 583.634 & 100 & 100 & 100\\
     281 & 732.419 & 750.579 & 100 & 100 & 100\\
     283 & 769.997 & 733.641 & 100 & 100 & 100\\
     293 & 909.637 & 888.776 & 100 & 100 & 100\\ 
     \hline
     401 & 345600* & 0.12256* & 100 & 65 & 100\\
     \end{tabular}
    \end{table}
